Offline Imitation from Observation via Primal Wasserstein State Occupancy Matching

In real-world scenarios, arbitrary interactions with the environment can often be costly, and actions of expert demonstrations are not always available. To reduce the need for both, offline Learning from Observations (LfO) is extensively studied: the agent learns to solve a task given only expert states and task-agnostic non-expert state-action pairs. The state-of-the-art DIstribution Correction Estimation (DICE) methods, as exemplified by SMODICE, minimize the state occupancy divergence between the learner's and empirical expert policies. However, such methods are limited to either $f$-divergences (KL and $chi^2$) or Wasserstein distance with Rubinstein duality, the latter of which constrains the underlying distance metric crucial to the performance of Wasserstein-based solutions. To enable more flexible distance metrics, we propose Primal Wasserstein DICE (PW-DICE). It minimizes the primal Wasserstein distance between the learner and expert state occupancies and leverages a contrastively learned distance metric. Theoretically, our framework is a generalization of SMODICE, and is the first work that unifies $f$-divergence and Wasserstein minimization. Empirically, we find that PW-DICE improves upon several state-of-the-art methods. The code is available at https://github.com/KaiYan289/PW-DICE.

==> backup-latex-files/backup-Methodology.tex <==
\section{Method}
\label{sec:method}

This section is organized as follows: in Sec.~\ref{sec:method_motivation}, we first validate our motivation, i.e., the importance of selecting an adequate distance metric by comparing metrics using existing Wasserstein-based solutions; then, we detail our proposed optimization objective in Sec.~\ref{sec:reg}; before converting it into a single-level convex optimization in Sec.~\ref{sec:fenchel}; finally, we discuss our choice of distance metric in Sec.~\ref{sec:contra}. See Tab.~\ref{tab:notelist} in Appendix~\ref{sec:notlist} for a reference of the notation.

\subsection{Validation of Motivation}
\label{sec:method_motivation}
% for better readability, we assume S is finite and the minimum value is reachable (inf->min); the idea is the same

As mentioned in Sec.~\ref{sec:intro}, our goal is to improve the idea of divergence minimization between the learner's policy and the expert policy estimated from the expert dataset. For this we suggest to use the primal Wasserstein distance with arbitrary underlying distance metric. To better show the importance of distance metrics and the advantage of being able to select them, we study Optimal Transport Reward (OTR)~\cite{luo2023otr}, a current Wasserstein-based IL method that can be applied to our LfO setting. OTR optimizes the primal Wasserstein distance between every trajectory in the task-agnostic dataset and the expert trajectory, and uses the result to assign a reward to each state in the task-agnostic dataset; then, offline RL is applied to retrieve the optimal policy. Fig.~\ref{fig:motivation} shows results of OTR on the D4RL MuJoCo dataset (see Sec.~\ref{sec:MuJoCoexp} for more) with testbeds appearing in both SMODICE~\cite{ma2022smodice} and OTR; we test both the cosine-similarity-based occupancy used in the paper and Euclidean distance as the underlying distance metric. The result illustrates that distance metrics have a significant impact on results; thus, a good metric is crucial for the performance of Wasserstein-based solutions.  

This experiment motivates our desire to develop a method that permits use of arbitrary distance metrics in Wasserstein-based formulations; further, the performance difference inspires us to automate selection of the metric and go beyond simple, heuristic metrics such as cosine and Euclidean. We discuss the formulation of our suggested method next.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{pic/OTRtest-partial.png}
    \caption{Performance comparison between OTR~\cite{luo2023otr} with default distance metric and Euclidean distance metric on OTR (first column) and SMODICE~\cite{ma2022smodice} (second and third column) settings. The result shows that the underlying distance metric is crucial to the performance of Wasserstein-based method.}
    \label{fig:motivation}
\end{figure}

\subsection{Optimization Objective}
\label{sec:reg}

Our goal is to optimize the primal Wasserstein distance between the model-estimated state occupancy $d^\pi_s(s)$ induced by the policy $\pi$ and the empirical state occupancy  $d^E_s(s)$ estimated from expert data. 
This can be formalized via the following program: 
\begin{equation}
\min_{\Pi, \pi}\sum_{s_i\in S}\sum_{s_j\in S}\Pi(s_i, s_j)c(s_i,s_j), \text{s.t. }  d^\pi_{sa}\geq 0, \Pi\geq 0; 
\label{eq:primal_main}
\end{equation}
\begin{gather*}
\small
\forall s\in S, d^\pi_s(s)=(1-\gamma)p_0(s)+\gamma\sum_{\bar{s},\bar{a}}d^\pi_{sa}(\bar{s},\bar{a})p(s|\bar{s},\bar{a});\\
\forall s_i, s_j\in S,\sum_k\Pi(s_k, s_j)=d^E_s(s_j), \sum_k\Pi(s_i,s_k)=d^\pi_s(s_i).
\end{gather*}
In Eq.~\eqref{eq:primal_main}, we use $\Pi(s_i, s_j)$ as the matching variable between two state distributions, and $c(s_i, s_j)$ is the distance between states $s_i$ and $s_j$. 
%$d^E_s$ is the state occupancy of the expert policy, $d^\pi_s$ is the state occupancy induced by policy $\pi$, and 
$d^\pi_{sa}$ is the state-action occupancy of our learned policy $\pi$, and $p_0\in\Delta(S)$ is the distribution of the MDP's initial states. Note that there are two types of constraints in Eq.~\eqref{eq:primal_main}: the first row, together with $d^\pi_{sa}\geq 0$, is the marginal constraint for the matching variable $\Pi$. The second row and $\Pi\geq 0$ are the \textit{Bellman flow constraints}~\cite{ma2022smodice} that ensure correspondence between $d^\pi_s$ and a feasible policy $\pi$.

For a tabular MDP, Eq.~\eqref{eq:primal_main} can be solved by any Linear Programming (LP) solver, as both the objective and the constraints are linear. However, using an LP solver is impractical for any MDP with continuous state or action spaces. In these cases, we need to convert the problem into an unconstrained optimization that is easy to optimize, and prefereably single-level to avoid instability in iterations. Before doing so,
%Thus, we will add a pessimistic regularizer in Sec.~\ref{sec:reg} to Eq.~\eqref{eq:primal_main}, with which the Lagrange dual of the problem is unconstrained. We derive the closed-form solution and retrieve policy in Sec.~\ref{sec:fenchel}, and discuss the distance metric selection in Sec.~\ref{sec:contra}.
for  readability, we rewrite our main objective in Eq.~\eqref{eq:primal_main} as an LP problem over a single vector $x=\begin{bmatrix}\Pi\\d^\pi_{sa}\end{bmatrix}\in\mathbb{R}^{|S|\times(|S|+|A|)}$, where $\Pi\in\mathbb{R}^{|S|\times|S|}$ and $d^\pi_{sa}\in\mathbb{R}^{|S|\times|A|}$ are flattened in a row-first manner. Correspondingly, we extend the distance $c$ between states to $c': (|S|(|S|+|A|))\times (|S|(|S|+|A|))\rightarrow\mathbb{R}$, such that $c'=c$ on the original domain of $c$ and $c'=0$ otherwise. Further, we summarize all linear equality constraints in $Ax=b$.  Eq.~\eqref{eq:primal_main} is then equivalent to
\begin{equation}
\min_{x\geq 0} (c')^Tx \quad\text{s.t.}\quad Ax=b, x\geq 0.
\label{eq:simplify}
\end{equation}
%Here, $b=\begin{bmatrix}-(1-\gamma)p_0\\0\\d^E_s\end{bmatrix}$ (see Sec.~\ref{sec:fenchel} for the elements of $A$.) 
It is easy to see that the Lagrange dual form of Eq.~\eqref{eq:simplify} is also a constrained optimization. %In order to remove the constraints in the dual
In order to convert the optimization to an unconstrained one, we modify the objective as follows:
\begin{equation}
\min_x (c')^Tx+\epsilon_1 D_f(\Pi\|U)+\epsilon_2 D_f(d^\pi_{sa}\|d^I_{sa}), \text{s.t. } Ax=b, x\geq 0,
\label{eq:reg}
\end{equation}
where $U(s,s')=d^E_s(s)d^I_s(s')$, i.e., $U$ is the product of two independent distributions $d^E_s$ and $d^I_s$. $\epsilon_1>0, \epsilon_2>0$ are hyperparameters, and $D_f$ can be any $f$-divergence. Note though $f$-divergence is used, unlike SMODICE~\cite{ma2022smodice} or LobsDICE~\cite{Kim2022LobsDICEOL}, such formulation does not require data coverage of the task-agnostic data over expert data. The two regularizers are ``pessimistic'', which encourages the agents to stay within the support set of the dataset and is common in offline IL/RL~\cite{jin2021pessimism}. 
With the regularized objective in Eq.~\eqref{eq:reg}, we now consider its Lagrange dual problem:
\begin{equation}
\begin{aligned}
\label{eq:lag1}
\max_\lambda\min_{x\geq 0}L(\lambda, x),\text{ where }
L(\lambda, x)=(c')^Tx+\\\epsilon_1D_f(\Pi\|U)+\epsilon_2D_f(d^\pi_{sa}\|d^I_{sa})-\lambda^T(Ax-b).
\end{aligned}
\end{equation}


% is row-first clear enough?

\subsection{Convertion Into Single-Level Convex Optimization}
\label{sec:fenchel}

While Eq.~\eqref{eq:lag1} is unconstrained, it is a bi-level optimization; to obtain a practical and stable solution, a single-level optimization is preferred. To do so, one could consider using the KKT condition~\cite{boyd2004convex}, and set the derivative of the inner-level optimization to $0$; however, such approach will lead to an exp function in the objective~\cite{MITnote, Kim2022LobsDICEOL}, which is numerically unstable~\cite{Kim2022LobsDICEOL}. To avoid this, we first rewrite Eq.~\eqref{eq:lag1} \textit{with negated $L(\lambda, x)$} to separate $\Pi$ and $d^\pi_{sa}$ in $x$:

\begin{equation}
\small
\begin{aligned}
\label{eq:separate}
\min_\lambda &\{\epsilon_1\max_{\Pi\in\Delta(S^2)}[\frac{(A_1^T\lambda-c)}{\epsilon_1}^T\Pi-D_f(\pi\|U)]\\&+\epsilon_2\max_{d^\pi_{sa}\in\Delta(S\cdot A)}[\frac{(A_2^T\lambda)}{\epsilon_2}^Td^\pi_{sa}-D_f(d^\pi_{sa}\|d^I_{sa})]-b^T\lambda\}.    
\end{aligned}
\end{equation}

In Eq.~\eqref{eq:separate}, we have $A=\begin{bmatrix}A_1\\A_2\end{bmatrix}$, where $A_1\in\mathbb{R}^{(|S|\times|S|)\times M}$, $A_2\in\mathbb{R}^{(|S|\times|A|)\times M}$, and $M=3|S|$ is the number of equality constraints in the primal form. There are two things worth noting in Eq.~\eqref{eq:separate}. First, we append two extra constraints, which are $\Pi\in\Delta, d^\pi_{sa}\in\Delta$. Such appended constraints does not affect final results for the following fact:

\begin{lemma}
\label{thm:lemma}
For any MDP and feasible expert policy $\pi^E$, the inequality constraints in Eq.~\eqref{eq:primal_main} with $\Pi\geq 0, d^\pi_{sa}\geq 0$ and $\Pi\in\Delta, d^\pi_{sa}\in\Delta$ are equivalent.
\end{lemma}

The detailed proof of Lemma~\ref{thm:lemma} is given in the Appendix~\ref{sec:invariance}; in a word, the optimal solution of Eq.~\eqref{eq:lag1}, as long as it satisfies all constraints in the primal form, must have $\Pi\in\Delta, d^\pi_{sa}\in\Delta$. Second, we decompose the max operator into two independent maximizations, as the equality constraints that correlate $\Pi$ and $d^\pi_{sa}$ are all relaxed in the dual.%, and $b^T\lambda$ is independent from the maximization. 
% warning: add this in the appendix!
 With Eq.~\eqref{eq:separate}, we now apply the following theorem from  SMODICE~\cite{ma2022smodice}:

\begin{theorem} % space-saving version
\label{thm:smodice}
With mild assumptions~\cite{pmlr-v54-dai17a}, for any $f$-divergence $D_f$, probability distribution $p,q$ on domain $\mathcal{X}$ and function $y: \mathcal{X}\rightarrow\mathbb{R}$, we have

\begin{equation}
\small
\max_{p\in\Delta(\mathcal{X})}\mathbb{E}_{x\sim p}[y(x)]-D_f(p\|q)=\mathbb{E}_{x\sim q}[f_*(y(x))].
\end{equation}

For maximizer $p^*(x)=\mathop{\arg\max}_{p\in\Delta(\mathcal{X})}\mathbb{E}_{x\sim q}[f_*(y(x))]$, we have $p^*(x)=q(x)f'_*(y(x))$, where $f_*(\cdot)$ is the Fenchel conjugate of $f$, and $f'_*$ is its derivative.
\end{theorem}

% \begin{theorem}
% \label{thm:smodice}
% With mild assumptions~\cite{pmlr-v54-dai17a}, for any $f$-divergence $D_f$, probability distribution $p,q$ on domain $\mathcal{X}$ and function $y: \mathcal{X}\rightarrow\mathbb{R}$, we have

% \begin{equation}
% \small
% \max_{p\in\Delta(\mathcal{X})}\mathbb{E}_{x\sim p}[y(x)]-D_f(p\|q)=\mathbb{E}_{x\sim q}[f_*(y(x))]
% \end{equation}

% also, for $p^*=\mathop{\arg\max}_{p\in\Delta(\mathcal{X})}\mathbb{E}_{x\sim q}[f_*(y(x))]$, we have 
% \begin{equation}
% \small
% p^*(x)=q(x)f'_*(y(x)),
% \end{equation}
% where $f_*(\cdot)$ is the Fenchel conjugate of $f$, and $f'_*$ is its derivative.
% \end{theorem}

A complete proof can be found at theorem $7.14^*$ in~\cite{MITnote}, and the theorem is discussed in the Appendix~\ref{sec:thm1}. The rigorous notion of $f$-divergence and Fenchel conjugate are in the Appendix~\ref{sec:mathcon}. For this work, we mainly consider KL-divergence as $D_f$, which corresponds to $f(x)=x\log x$, and $f_*(x)=\text{logsumexp}(x)$ to be the Fenchel dual function with $x\in\Delta$~\cite{boyd2004convex}. \footnote{$\chi^2$-divergence does not work as well as KL-divergence in MuJoCo environment; see Appendix~\ref{sec:chidiv} for details.} With Thm.~\ref{thm:smodice}, we set $p=\Pi, x=\lambda, y(x)=\frac{A_1^T\lambda-c}{\epsilon_1}$ for the first max operator, and set $p=d^\pi_{sa}, x=\lambda, y(x)=\frac{A_2^T\lambda}{\epsilon_2}$ for the second max operator. Then, we get the following single-level convex objective:

\begin{equation}
\begin{aligned}
\label{eq:singlelevel}
\small
\min_\lambda &\epsilon_1 \log\mathbb{E}_{s_i\sim I, s_j\sim E}\exp(\frac{(A_1^T\lambda-c)^T}{\epsilon_1})\\&+\epsilon_2\log\mathbb{E}_{(s_i,a_j)\sim I}\exp(\frac{A^T_2\lambda}{\epsilon_2})-b^T\lambda.
\end{aligned}
\end{equation}


Finally, by considering the elements in $A$ (see Appendix~\ref{sec:component}), we get our final objective

\begin{equation}
\small
\begin{aligned}
\label{eq:final}
\min_\lambda&\ \epsilon_1\log \mathbb{E}_{s_i\sim I, s_j\sim E}\exp(\frac{\lambda_{i+|S|}+\lambda_{j+2|S|}-c(s_i,s_j)}{\epsilon_1})+\\
\epsilon_2\log &\mathbb{E}_{(s_i,a_j)\sim I}\exp(\frac{-\gamma \mathbb{E}_{s_k\sim p(\cdot|s_i,a_j)}\lambda_k+\lambda_i-\lambda_{i+|S|}}{\epsilon_2})\\&-[(1-\gamma)\mathbb{E}_{s\sim p_0}\lambda_{:|S|}+\mathbb{E}_{s\sim E}\lambda_{2|S|:3|S|}],
\end{aligned}
\end{equation}

where $d^\pi_{sa}=d^I_{sa}\cdot \text{softmax}(\frac{-\gamma \mathbb{E}_{s_k\sim p(\cdot|s_i,a_j)}\lambda_k+\lambda_i-\lambda_{i+|S|}}{\epsilon_2})$ at optimal, and the denominator of the softmax is summing over all state-action pairs. Thus, we can now retrieve the desired policy $\pi$ by weighted behavior cloning:

\begin{equation}
\small
\begin{aligned}
\label{eq:policy}
&\mathbb{E}_{(s_i,a_j)\sim d^\pi_{sa}}\log p(a|s)=\mathbb{E}_{(s_i,a_j)\sim I}\frac{d^\pi_{sa}(s_i,a_j)}{d^I_{sa}(s_i,a_j)}\log p(a_j|s_i)\\
\propto& \mathbb{E}_{(s_i,a_j)\sim I}\exp(\frac{-\gamma \mathbb{E}_{s_k}\lambda_k+\lambda_i-\lambda_{i+|S|}}{\epsilon_2})\log p(a_j|s_i).
\end{aligned}
\end{equation}
In practice, we use $1$-sample estimation for $p(\cdot|s_i, a_j)$, which is found in prior works to be simple and effective~\cite{ma2022smodice, Kim2022LobsDICEOL}. That is, we sample $(s_i,a_j,s_k)\sim I$ from the dataset instead of $(s_i, a_j)$, and use $\lambda_k$ corresponding to $s_k$ as an estimation for $\mathbb{E}_{s_k\sim p(\cdot|s_i,a_j)}\lambda_k$. Since the number of states can be infinite in practice, we use a 3-head neural network to estimate $\lambda_s, \lambda_{s+|S|}$ and $\lambda_{s+2|S|}$ given state $s$.

Note, the formulation can be seen as a generalization of SMODICE~\cite{ma2022smodice}. More specifically, we have the following theorem (see Appendix~\ref{sec:proof} for proof):

\begin{theorem}
\label{thm:general}
If $c(s_i,s_j)=-\log\frac{d^E_s(s_i)}{d^I_s(s_i)}, \epsilon_2=1$, then as $\epsilon_1\rightarrow 0$, Eq.~\eqref{eq:final} is equivalent to SMODICE objective with KL divergence.  
\end{theorem}

For different $D_f$, similarly we have the following corollary:

\begin{corollary}
\label{thm:corol}
If $c(s_i,s_j)=-\log\frac{d^E_s(s_i)}{d^I_s(s_i)}, \epsilon_2=1$, then as $\epsilon_1\rightarrow 0$, Eq.~\eqref{eq:separate} is equivalent to SMODICE with any $f$-divergence.
\end{corollary}
Thus, our PW-DICE work is a unification of $f$-divergence and Wasserstein distance minimization.

\subsection{Underlying Distance Metric}
\label{sec:contra}

With Eq.~\eqref{eq:final} and~\eqref{eq:policy}, the only problem remaining is to choose the distance metric $c(s_i, s_j)$. For tabular cases, one could use the simplest distance, i.e., $c(s_i,s_j)=1$ if $s_i\neq s_j$, and $0$ otherwise. However, such design would lead to gradient disappearance in continuous case; to address this, prior works have explored many heuristic choices, such as cosine similarity~\cite{luo2023otr} or Euclidean~\cite{sun2021softdice}. However, such heuristic choice is prone to different representations over the same state. 

In this work, inspired by both CURL~\cite{laskin2020curl} and SMODICE~\cite{ma2022smodice}, we propose a weighted sum of $R(s)=\log\frac{d^E_s(s)}{(1-\alpha)d^I_s(s)+\alpha d^E_s(s)}$ and the Euclidean distance between an embedding learned by the InfoNCE~\cite{infonce} loss. To be more specifically, we have    $c(s_i,s_j)=R(s_i)+\beta\|g(s_i)-g(s_j)\|^2_2$,
where $g(s_i), g(s_j)$ are embeddings for the states $s_i, s_j$, $\alpha$ is a positive constant close to $0$, and $\beta\geq 0$ is a hyperparameter. 

The distance function consists of two parts. The first part, $R(s_i)$, is an improved version of reward function $\log\frac{d^E_s(s)}{d^I_s(s)}$ in SMODICE~\cite{ma2022smodice}; intuitively, high $\log\frac{d^E_s(s)}{d^I_s(s)}$ indicates that the state $s$ is more frequently visited by the expert than agents generating the task-agnostic data, which is probably desirable. Such reward can be obtained by training a discriminator $c(s)$ that takes expert states from $E$ as label $1$ and non-expert ones as label $0$. If $c$ is optimal, i.e., $c(s)=c^*(s)=\frac{d^E_s(s)}{d^E_s(s)+d^I_s(s)}$, then we have $\frac{d^E_s(s)}{d^I_s(s)}=\log\frac{c^*(s)}{1-c^*(s)}$. We change the denominator $d^E_s(s)$ to $(1-\alpha)d^I_s(s)+\alpha d^E_s(s)$ to lift the theoretical assumption that the task-agnostic dataset $I$ covers the expert dataset $E$, i.e., $d^I_s(s)>0$ wherever $d^E_s(s)>0$. 

The second part uses embedding $g(s)$ learned with infoNCE~\cite{infonce} following CURL~\cite{laskin2020curl}, such that $g(s)$ and $g(s')$ are similar if and only if they can be reachable along trajectories in the task-agnostic dataset. 
%More specifically, we use the following loss function:
% \begin{equation}
% \label{eq:infonce}
% L_c=\log\frac{\exp(q^TWk_+)}{\exp(q^TWk_+)+\sum_{k_-}\exp(q^TWk_-)},
% \end{equation}
% where $q$ is the query (anchor), $W$ is a learned, semi positive-definite weight matrix, $k_+$ is positive key, and $k_-$ are negative keys. To train the embedding function $f$, for every gradient step, we sample a batch of adjacent state pairs $\{(s_i, s'_i)|i\in\{1,2,\dots, K\}\}$; then, for $q=f(s_i)$, we set $k_+=f(s'_i)$ and the set of $k_-$ to be $\{f(s'_j)|j\neq i\}$; this essentially amounts to a $K$-way classification task, where for the $i$-th sample the correct label is $i$. 
Intuitively, the idea is to learn a good embedding space where the vicinity of state can be evaluated by the Euclidean distance between the embedding vectors. We define the vicinity as the ``reachability'' between states; that is, if one state can reach the other through a trajectory in the task-agnostic data, then they should be close; otherwise, they are far away. Such definition clusters states that lead to success together in the embedding space, while being robust to actual numerical values of the state. See Appendix~\ref{sec:expdetail} for details and Appendix~\ref{sec:robust} for empirical validation.



